Vision-Language Instruction Tuning: A Review and Analysis

Instruction tuning is a crucial supervised training phase in Large Language Models (LLMs), aiming to enhance the LLM's ability to generalize instruction execution and adapt to user preferences. With the increasing integration of multi-modal data into LLMs, there is growing interest in Vision-Language Instruction Tuning (VLIT), which presents more complex characteristics compared to pure text instruction tuning. In this paper, we systematically review the latest VLIT settings and corresponding datasets in multi-modal LLMs and provide insights into the intrinsic motivations behind their design. For the first time, we offer a detailed multi-perspective categorization for existing VLIT datasets and identify the characteristics that high-quality VLIT data should possess. By incorporating these characteristics as guiding principles into the existing VLIT data construction process, we conduct extensive experiments and verify their positive impact on the performance of tuned multi-modal LLMs. Furthermore, we discuss the current challenges and future research directions of VLIT, providing insights for the continuous development of this field. The code and dataset related to this paper have been open-sourced at https://github.com/palchenli/VL-Instruction-Tuning.

==> section/old2.tex <==
\section{What Does High-Quality VLIT Data Look Like?}\label{sec:method}

In this section, we'll tackle the first problem first.
Specifically, we summarize the characteristics that high-quality VLIT data should have, as discussed in the above works, and generalize them into a set of complete basic principles for VLIT construction and evaluation. 

\subsection{Characteristics and Principles}\label{sec:principle}

\subsubsection{Diversity}

Diversity has long been a focal point for natural language generation and a crucial aspect in evaluating content quality~\citep{evaldis2020arxiv,evaldis22020arxiv}. 
Especially in the tuning of LLM instructions, diversity plays a crucial role in determining the capability of LLM to generalize instructions~\citep{zhang2023instruction}. 
Specifically, within the domain of VLIT, diversity demonstrates distinct characteristics, predominantly manifested in three areas:

\paragraph{Task Diversity.}

Whether using LLM or MLLM, the quantity of task clusters has always been a critical focus in the creation of instruction-following data. 
This is because LLM must be exposed to an adequate number of tasks to possess the ability to generalize and implement instructions. 
In the multi-modal scene, presented in Table~\ref{tab:ds_task} in the appendix, existing MLLM encompasses a considerable amount of visual tasks. 
In order to further enrich the task types, a large number of MLLM also incorporate pure text instruction data into VLIT data (e.g., mPLUG-Owl and MultiModal-GPT), which has achieved positive improvements.

\paragraph{Instruction Diversity.}

Unlike the execution of a singular task, existing works usually form a small-scale (five to ten or more) candidate instruction pool manually while assigning corresponding instructions for a specific task to enhance the tuned LLM's instruction generalization capabilities~\citep{mini42023arxiv,instructblip2023arxiv}.
Subsequently, while constructing instruction-response pairs, varied pairing schemes can be attained by choosing instruction texts and responses randomly from the candidate instruction pool. 
As the LLM becomes more advanced, some methods will choose to use LLM (e.g., ChatGPT, GPT-4, and LLaMA) further to expand the size of the candidate instruction pool, and even guide the LLM to generate natural language instructions autonomously in the way of in-context learning~\citep{mimic2023arxiv}. 
The above operations all show that the instructions corresponding to each task in the VLIT data also need to be diverse, otherwise, problems such as over-fitting and poor generalization will greatly affect the performance of MLLM in downstream tasks, especially in the zero-shot setting.

\paragraph{Response Diversity.}

Furthermore, responses with greater diversity have the potential to enhance user experience and satisfaction in response to input content and instructions.
Therefore, in addition to simply rewriting the response text, to further improve the semantic information scale of the response text, some works summarize different types of annotation data of the same sample together to further improve the possibility of generated VLIT data~\citep{llava2023arxiv}.
In addition, some researchers~\citep{ferret2023arxiv,lrv2023arxiv} find that it is not enough for MLLM to understand positive samples to improve its discrimination ability, so they generate a large number of negative samples for tasks such as visual question-answering to further improve the overall diversity.
However, due to the large scale of data and insufficient annotation, the above problems are often ignored in current research.

\subsubsection{Complexity}

The introduction of visual information in MLLMs greatly increases the difficulty of content understanding. 
On the one hand, this is manifested in the fact that the information objects that MLLMs need to understand become more complex and diverse. 
On the other hand, this is manifested in the increased complexity of instruction and content logic itself.

\paragraph{Object/Granularity Complexity.}

In the field of multi-modal analysis, visual input, along with text, is the most widespread source of information.
However, as a common analog signal, images contain semantic information of different granularities.
The complexity of objects comes from this. 
The introduction of visual objects of different granularities (even resolution ratio) and interaction with text information can significantly improve the ability of MLLM to process information~\citep{nextgpt2023arxiv,anymal2023arxiv}.
Therefore, the complexity of the objects involved in the instruction data is something that must be considered in constructing high-quality VLIT data.

\paragraph{Instruction Complexity.}

In its early days, the instruction tuning mechanism was primarily adapted from common visual tasks, making instructions simple to carry out. 
As demands have grown for more varied tasks such as complex reasoning and user preference adaptation, instruction complexity has increased. 
At the same time, some detailed designs combined with real application scenarios also increase the complexity of instructions, such as: "brief answer" and "in detail".
These complex instructions can guide MLLM to complete more difficult tasks, thereby improving MLLM's problem-solving capabilities.
In particular, Chain-of-Thought~\citep{cot2022arxiv} is a setting that assists MLLM in solving such complex problems, and accordingly, the concept of COT tuning is proposed.

\subsubsection{Balance}

The maintenance of data balance is crucial in both traditional machine learning model training and LLMs. 
Research indicates that uneven data settings or large-scale supervised fine-tuning may lead to forgetting phenomena in large models, significantly impeding their overall performance~\citep{instructionminigpt2023arxiv,forget2023arxiv}. 
Therefore, recent research highlights the importance of enhancing the consideration of data (task) balance in construction and training processes.

\section{How to Construct High-Quality VLIT Data}\label{sec:vlit_pipeine}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/fig_const_pipeline.pdf}
    \caption{VLIT Dataset Construction Pipeline.}
    \label{fig:const_pipeline}
\end{figure}

In this section, we focus on the second problem, and we synthesize the refined characteristics of high-quality VLIT data and propose the complete VLIT data construction pipeline, as shown in Figure~\ref{fig:const_pipeline}.
On this basis, we collect rich real annotation data, implement corresponding functional modules in the proposed pipeline, and finally give a feasible implementation method and an example VLIT dataset.

\subsection{Construction Pipeline}

In order to ensure the quality of the constructed VLIT data, the principles summarized in Section~\ref{sec:principle} need to be considered both when generating instruction-response pairs and after generating them.

\subsubsection{Data Collection}

Multi-modal annotation data, which is utilized to generate VLIT data, typically derives from various visual tasks, including recognition, segmentation, etc. 
These tasks commonly act as sources of supervision for training traditional machine learning models and offer high-quality data at a significant scale, rendering them highly practical. 

When collecting data, it is necessary to pay attention to some elements such as annotation data type, source, scale, and quality, which can ensure the diversity and complexity of the VLIT data for the collected information.
Specifically, firstly, different annotation data types are usually linked to various task types, which can greatly enhance the diversity of the final VLIT data.
Second, when multi-modal data from the same source contains diverse types of annotations, it can generate more complex contexts and task types on top of the original simple vision task ~\citep{llava2023arxiv}.
Again, although the amount of instruction data may not scale steadily with the performance of an MLLM, large-scale MLLMs with many parameters require adequate data scale ~\citep{instructgpt2022nips}.
Finally, according to the~\citeauthor {instructionminigpt2023arxiv} the maturing of the conclusion, the size of the data must be considered when collecting data, and quality to achieve the balance.
In addition, in addition to the initial annotation data, the plain text instruction set of existing multi-modal instructions should also be collected as valuable data that can be directly reused.

\subsubsection{Instruction-Response Generation}

Currently, the use of LLM (e.g., ChatGPT, GPT4, and LLaMA) to aid in generating VLIT data is well established, and thus we directly reuse the existing VLIT generation mode~\citep{llava2023arxiv}. 
Specifically, when provided with an image $img$ and corresponding annotation data of various types $\{Anno_{1}, Anno_{2}, ..., Anno_{n}\}$, appropriate templates are manually designed for each type of annotation data to ensure the annotated data conforms to standard language representation after insertion. 
After combining all sources of annotation data, a highly detailed description of an image can be obtained, which is the comprehensible visual clue for a language-only LLM.

To ensure correct and stable generation of the required content, a prompt text must be written to guide LLM, and a small number of example instruction-response pairs need to be manually written for in-context learning under different requirements.
In the system prompt design, we follow the principles proposed in Section~\ref{sec:principle} and input specific prompts (e.g., extended knowledge, negative sample, multi-round conversation, etc.)\footnote{Please refer to Section~\ref{sec:sp} in Appendix.} to guide the generator to generate more diverse and complex instruction-response pairs.
At the same time, the in-context examples\footnote{Please refer to Section~\ref{sec:ice} in Appendix.} we designed should meet the characteristics of comprehensiveness and randomness, corresponding to the boundaries involved and providing appropriate examples for all possible scenarios, so that the generator can correctly understand the meaning of the prompts.
In addition, based on established experience, we also set redundancies in the key points of system prompts and in-context examples.

At this point, language-only LLM can realize the generation of instruction-response pairs based on the above three kinds of information, i.e., visual clues, system prompts, and in-context examples.

\subsubsection{Quality Control}\label{sec:qc}

Due to the possibility of errors in LLM itself and the uncontrollable distribution of generated data, it is necessary to perform quality control on the VLIT data directly output by LLM. 
Recently, many works have begun to pay attention to this issue and have filtered data based on some mature experiences~\citep{mimic2023arxiv,m3it2023arxiv}.
In this paper, we have designed corresponding data filtering strategies for the characteristics of high-quality VLIT data proposed in section~\ref{sec:principle}, and conducted local and global quality control on the generated VLIT data. 

Specifically, for each VLIT sample, we evaluate its quality from the following two perspectives:

\begin{itemize}
    \item \textbf{Matching Degree.} The generated VLIT data should have a high degree of matching with the original image.
    \item \textbf{Correctness.} Since the wrong instruction-response pairs can mislead the LLM, it is essential to ensure that the generated instruction-response pair is correct for the data.
\end{itemize}

In the overall evaluation of the VLIT data, we consider the three perspectives presented in Section~\ref{sec:principle}:

\begin{itemize}
    \item \textbf{Diversity.} Since the diversity of VLIT is reflected in three perspectives, its evaluation needs to examine three indicators: the number of task types, the similarity of instructions in each task, and the similarity of all response texts.
    \item \textbf{Complexity.} The complexity evaluation needs to refer to two objects: the occurrence distribution of different granularity information and the overall difficulty distribution of instructions.
    \item \textbf{Balance.} The balance of VLIT data mainly lies in measuring whether the distribution of different task types in the data is balanced, that is, whether there is a long tail.
\end{itemize}

\subsection{An Example Implementation}\label{sec:example_dataset}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figure/fig_example_pipeline.pdf}
    \caption{VLIT data generation data flow diagram based on GPT-3.5.}
    \label{fig:example_pipeline}
\end{figure}

In this paper, we provide a simple implementation based on the above pipeline to quickly construct VLIT data, as shown in Figure~\ref{fig:example_pipeline}.

\paragraph{Data Collection.} Specifically, we first select COCO 2014~\citep{coco2014eccv} as the image source, and $\{caption, object, attribute, OCR, visual QA\}$ as the selected sources of annotation data~\citep{cocovqa2015iccv,cocoattr2016eccv,cocotext2016arxiv}. 

\paragraph{Instruction-Response Generation.} We employ GPT-3.5~\citep{chatgpt} as the generator for LLM, and formulate corresponding system cues and in-context examples\footnote{See the Appendix for all system prompts used during the generation process}.
Specifically, based on the annotated data and different system prompts, we introduce different granularities of tasks, add negative samples, generate multi-turn complex dialogues, and extend external knowledge in the generation process to enhance the diversity and complexity of the generated VLIT data.
In addition, to further enhance diversity, we set the temperature value of GPT-3.5 to 0.8 and the number of generations to 5.

\paragraph{Quality Control.} Combining the quality control methods proposed in Section~\ref{sec:qc}, we choose CLIP~\citep{clip2021icml} as the vision-language pre-training model for evaluating the matching degree and LLaMA-2~\citep{llama-22023arxiv} as the LLM for evaluating the correctness of the generated instruction-response pair.
Specifically, we use the text encoder and image encoder in the tuned CLIP to encode the text guided by "This is a picture about this conversation:" and image respectively, and calculate the similarity between them as the matching degree score. 
The specific formula is as follows:
\begin{equation}
    score_{md} = \frac{v_{text} \cdot v_{image}}{||v_{text}|| \cdot ||v_{image}||}
\end{equation}
When evaluating the correctness, we take the detailed description used in the generation and the generated instruction-response pairs as input, use LEMA-2 to evaluate the correctness under the guidance of some examples, and take the highest frequency of the three evaluation results as the result.

We use the zero-shot labeler TagGPT~\citep{taggpt2023arxiv} to assign task labels to each VLIT data sample.
Among them, TagGPT is a labeler that can be cold-started. 
It generates labels to samples by introducing the semantic understanding capability of LLM, retains high-quality labels based on indicators such as label coverage and redundancy, and finally assigns labels to samples.
In this paper, we use LLaMA-2 based Taggpt to target tasks and generate task labels for the generated VLIT data.
When evaluating instruction diversity, since there is still some semantic similarity in the instruction text for tasks with the same task type, it is not possible to directly use semantic calculations to evaluate instruction diversity. 
Although some methods try to avoid this problem by counting predicate verbs, some noun information also affects the calculation of diversity. 
In this paper, we use a graph-based method to calculate instruction diversity, namely, converting instruction texts with the same task label into an element graph based on co-occurrence relationships after removing stop words and using the overlapping community partitioning method (i.e., Ego-Splitting~\citep{ego-spl2017kdd}) to count the number of clusters to evaluate instruction diversity.
Ego-Splitting is a generative model with overlapping clusters in which it is able to reconstruct most of the clusters exactly by using the connected component algorithm as a non-overlapping partition algorithm both in the ego-net clustering phase and in the persona graph clustering phase.
When evaluating response diversity, we directly utilize an efficient unsupervised text representation method (i.e., SimCSE~\citep{simcse2021emnlp}) to represent response texts and employ a density-based clustering algorithm (i.e., DBScan~\citep{dbscan2017tods}) to mine semantic clusters as indicator.
SimCSE generates unsupervised positive samples by randomly sampling dropout masks to improve contrastive learning performance. 
That is, during the training phase, the same sample is input into the same encoder twice to obtain two different representation vectors $z, z'$, $z'$ will be used as a positive sample, then the training target of the model is:
\begin{equation}
    l_{i} = - \log \frac{\mathrm{e}^{sim(h_{i}^{z_{i}},h_{i}^{z'_{i}})/\tau}}{\sum_{j=1}^{N} \mathrm{e}^{sim(h_{i}^{z_{i}},h_{j}^{z'_{j}})/\tau}}.
\end{equation}
DBScan is a clustering method that treats clusters as dividing high-density areas by low-density areas in the data space, and divides sufficiently high-density areas into clusters.
It cycles through labeling candidate samples to corresponding clusters and deleting them, and finally achieves clustering after all samples are labeled.

In addition, to evaluate complexity, we first use classical semantic dependency analysis to count the number of elements in the instructions~\citep{srl2008cl}, and then utilize LLaMA-2 as the discriminative model to provide a quantitative difficulty score under the guidance of the given sample.
Specifically, semantic dependency analysis refers to the task of extracting important semantic elements in a text and assigning corresponding roles.
In this paper, we use mature tools\footnote{\url{https://hanlp.hankcs.com/demos/sdp.html}} for semantic role extraction as a data source for counting the number of instruction elements.
When evaluating the complexity of instructions, similar to existing work, we input given instruction-reply pairs into LLM and rely on manually scored examples to give all candidate pairs a complexity score of 1-10.

Finally, when evaluating balance, we can use the obtained task labels to calculate the variance of the number of samples in different tasks as the balance indicator.

==> section/ord1.tex <==
\input{table/fig_tree}
\input{table/tab_mllm}
\input{table/tab_dataset}

\subsection{Vision-Language Instruction Data}

As illustrated in Figure~\ref{fig:method_tree}, we organize all VLIT data-related work in this section. 
The specific statistical information of MLLMs and corresponding VLIT datasets can be found in Table~\ref{tab:mllm} and Table~\ref{tab:dataset}.
To divide the existing work in more detail, we divide all work into two categories: general instructions and specific instructions based on the different purposes of dataset construction.
Among them, general instructions refer to the constructed VLIT data that is not targeted at specific objects/tasks/domains and aims to consistently improve the generalization ability of tuned MLLM.
Specific instructions are specially constructed to fully consider the environment in which the tuned MLLM works and the data required to be handled.

\subsubsection{General Instruction}\label{sec:general_inst}

As shown in Figure~\ref{fig:inst_example}, the format of general VLIT data is similar to that of traditional pure text instruction data, which can be classified into different types depending on the construction paradigm.
Specifically, these paradigms can be divided into two major categories: Annotation Adaption and Self-Instruct.

\paragraph{Annotation Adaptation.}

In recent years, the burgeoning development of visual models has led to the emergence of large-scale, diverse, and high-quality annotated data, which is applicable to a plethora of downstream tasks and can be seamlessly tailored for use as instruction data. 
Numerous related studies, in particular, meticulously adapt the annotated data to conform to the $(\textit{Instruction}, \textit{Input}, \textit{Response})$ format featured in standard instruction data.  
The \textit{Instruction}, as a formal statement explaining the nature of the task, is directly obtained using manually written candidate instruction pools~\citep{mini42023arxiv,chatbridge2023arxiv}, while others~\citep{instructblip2023arxiv, videochat2023arxiv} use manual instructions as seeds to guide LLMs to expand the instruction pool and enrich instruction diversity. 
The \textit{Input} comprises images and optional context, typically sourced from the original annotation data, and forms a part of the entire instruction data. 
The \textit{Response} corresponds to the result found in the annotation data and is the output part of the instruction data. 
If the original annotation data fulfills the user's requirements, it is generally migrated without modification. 
However, it is important to note that for certain downstream tasks such as classification, judgment, and brief captions, which typically produce outputs of only words or short sentences, the original answer may need to be expanded based on input information using LLMs as necessary to avoid potential overfitting and other related issues. 
It is worth mentioning that certain studies view such concise responses as a form of instruction, and therefore, they opt to include appropriate limiting language in the instruction to address this issue~\citep{chatbridge2023arxiv}.

Among them, InstructBLIP~\cite{instructblip2023arxiv} mixes 10 types of visual tasks, carefully crafts several instruction templates, and adjusts corresponding instruction details based on the original task data, such as brief/short descriptions.
KOSMOS-2~\citep{kosmos22023arxiv} creates an instruction dataset based on collected grounded boxes and corresponding expressions, using existing instruction templates.
Based on a large number of image caption datasets, LMEye~\citep{lmeye2023arxiv} generates millions of large-scale VLIT datasets by using multiple-choice questions with correct and incorrect classification and one-in-four choice as the template for VLIT data generation.
MiniGPT-4~\citet{mini42023arxiv} utilizes its own pre-trained MLLM to produce a comprehensive description of an image, and then applies ChatGPT to revise the descriptions by removing any redundant information. After manual verification of the correctness of instruction data, the resultant VLIT data can be obtained, which is of high quality.
Lynx~\citep{lynx2023arxiv} collects tasks of 5 different modalities, and generates instruction-following data based on task instruction texts expanded with GPT-4~\citep{gpt42023arxiv}.
NExT-GPT~\citep{nextgpt2023arxiv} notices the lack of discussion on the diversity of input and output modalities in existing work on training data, and therefore proposes the T2M instruction dataset focusing on text2multi-modal instruction dataset.
DreamLLM~\citep{dreamllm2023arxiv} collects image-text pairs from MMC4~\citep{mmc42023arxiv} and LAION400M~\citep{laion2022arxiv}, and generates summaries and captions by utilizing GPT-4.
InternLM-XComposer~\citep{internlm2023arxiv} first generates a piece of text, and then adds the appropriate image to the corresponding position based on the degree of matching between the image and the text content, to generate image-text interleaved content instructions.
MiniGPT-v2~\citep{minigptv22023arxiv} follows the conversation template of LLaMA-2 and uses the task identification token to generate a large number of instruction templates for different tasks.

In general, Annotation Adaption is a fast and simple VLIT construction scheme, which can quickly convert annotation data into VLIT data, and expand VLIT data scale and task types at a low cost. 
However, its disadvantages are also obvious, such as poor diversity of instructions and responses, low sample utilization, and inability to adapt to user preferences.

\paragraph{Self-Instruct.}

The scale, diversity, and creativity of instructions are often limited by existing tasks and corresponding annotation data, impeding the universality of MLLMs adjusted through this data. 
The standard instruction format poses challenges in adapting to the changing real-world application scenarios and addressing user needs. 
Therefore, in order to obtain additional instruction data that is more applicable to real-world scenarios, Self-Instruct is commencing with~\citep{self-i2022arxiv} the introduction of more varieties of annotation data. 
This will aid LLMs in creating a greater diversity of instruction-following data that is richer in content. 

Specifically, such methods utilize the strong understanding and generation capabilities of LLMs. They bootstrap instruction data samples similar to manual examples, using in-context learning by manually producing a small number of high-quality examples as context. 
These data no longer have strict restrictions, allowing for greater diversity and complexity in both instructions and responses.

As a significant contribution to the field, LLaVA~\citep{llava2023arxiv} initiated the trend of leveraging LLM to construct general VLIT data by reorganizing existing annotation data.
Specifically, LLaVA guides GPT-4 or ChatGPT to generate high-quality multi-round discussions by providing image descriptions from multiple perspectives and bounding boxes specifying object locations. This approach can effectively prevent the lack of diversity and depth of inference caused by hasty and imprecise use of GPT-4 and annotation data to directly generate instructions.
Building upon LLaVA's inspiration, DetGPT~\citep{detgpt2023arxiv} directs ChatGPT to create Q\&A pairs through image captions, object categories, and predetermined prompts. ChatGPT uses in-context examples manually designed to ensure accuracy.
LAMM~\citep{lamm2023arxiv} defines multi-modal instruction-response pairs for four different scenarios, reorganizes publicly available annotated data using GPT-API, and generates diverse task instructions, forming conversation-style instruction data.
Following LLaVA's approach, SVIT~\citep{svit2023arxiv} gathers more data and creates an extensive instruction dataset while implementing quality control measures such as repetition, conversation rounds, and hallucination.
AnyMAL~\citep{anymal2023arxiv} adopts analogous methods proposed by LLaVA, utilizing Llama-2~\citep{llama-22023arxiv} to produce question-answer pairs for the provided image.
By writing in-context samples, StableLLaVA~\citep{stablellava2023arxiv} guides ChatGPT to generate images and corresponding dialogues. Different from other methods, the images in StableLLaVA are generated based on generation prompts and StableDiffusion images.
PVIT~\citep{pvit2023arxiv} presents a vision-language instruction dataset that aligns fine-grained regions with the caption, which is based on existing tasks and generates basic instruction data using predefined templates. Then, ChatGPT is used to rewrite the above content to add diversity and provide assurance for the quality of instruction-following data.
TextBind~\citep{textbind2023arxiv} collects a large number of image-text pairs from publicly available datasets, and generates instruction data by reorganizing the content using GPT4 after filtering and clustering.
Based on GPT, Sparkles~\citep{sparkles2023arxiv} generates a dataset containing two different types of instructions, corresponding to conceptual captions and visual genome, respectively.
Different from the above works, LVIS-INSTRUCT4V~\citep{gpt4v2023believe} uses the powerful visual understanding ability of the newly launched GPT-4V(ision)~\citep{gpt4v} to generate conversational question-answer pairs through self-reasoning and generate high-quality image captions guided by accurate bounding box information as instruction data.

Self-Instruct is a more flexible VLIT data construction scheme, which has the characteristics of high complexity, strong diversity, and excellent complexity, and gives MLLM a stronger ability to follow instructions and adapt to user needs. 
However, due to its extreme dependence on the ability of LLM to understand and organize the existing data, it not only has huge overhead, but also has the inherent hallucination of LLM, which also leads to the instability of the quality of the generated VLIT data.

\subsubsection{Specific Instruction}\label{sec:specific_inst}

The only difference between specific instructions and general instructions is whether they contain some designs oriented to specific needs (such as goals, tasks, and fields). 
Their construction solutions can also be divided into two categories: annotation adaptation and self-instruct.
To avoid possible confusion caused by multiple classifications, we only discuss the specific needs for which VLIT data is constructed in this section.

\paragraph{Object/Task-Specific Instruction.} 

To achieve more fine-grained multi-modal understanding, some MLLMs introduce more considerations to the understanding object when generating VLIT data.
Among them, GPT4RoI~\citep{gpt4roi2023arxiv} constructs end-to-end region-oriented instruction data based on publicly available datasets and preset single-region caption, multi-region captioning, single-region reasoning, and multi-region reasoning instruction data, with the region as the target.
ChatSpot~\citep{chatsopt2023arxiv} collects different task datasets for both global images and regions to enhance the model's ability to handle information at different granularities, and generates large-scale instruction-following data based on predefined instruction templates.
Ferret~\citep{ferret2023arxiv} focuses on regional spatial information that is ignored by the mainstream, and constructs regional information dialogues based on ChatGPT including a large number of negative samples.
VideoChat~\citep{videochat2023arxiv} adjusts narrative text for generating detailed video descriptions using GPT4, and generates question-and-answer conversations focused on temporal and causal factors using ChatGPT with video descriptions as the source of information.
VALLEY~\citep{valley2023arxiv} refers to LLaVA and VideoChat, and uses Stable-Vicuna to generate question-answer pairs and conversation data by synthesizing several publicly available visual causal inferences, character recognition, and video complex content understanding datasets.
ChatBridge~\citep{chatbridge2023arxiv} combines a large number of existing visual tasks and instruction data, and constructs more video-oriented sessions referring to the paradigm of LLaVA, forming a very large-scale instruction dataset MULTIS.
Video-ChatGPT~\citep{vidchatgpt2023arxiv} obtains a large number of video-detailed description pairs through manual annotation and a semi-automatic annotation framework based on existing multi-modal LLMs, and then uses GPT3.5 to assist in generating large-scale high-quality question-answer pairs.
Macaw-LLM~\citep{macaw2023arxiv} utilizes GPT-3.5 to assist in reorganizing manually annotated image and video captions based on predefined prompts, and generated instruction-following data.
LLaVAR~\citep{llavar2023arxiv} mainly focuses on text-rich image data, collects LAION-5B images containing text divides them into 14 clusters, and reorganizes them into large-scale noisy instructions and high-quality instructions based on whether GPT-4 is used.
Shikra~\citep{shikra2023arxiv} guides GPT-4 to generate question-answer pairs based on bounding boxes using publicly available object detection datasets.

\paragraph{Domain-Specific Instruction.}

In addition to strengthening the understanding of semantic information at different granularities, there are some MLLMs that focus more on the ability to solve problems in specific domains, so these MLLMs construct more VLIT data with domain features.
PMC-VQA~\citep{pmc-vqa2023arxiv} proposes a medical VLIT dataset, which generates 5 question-answer pairs about images by inputting image captions into ChatGPT, and designs to filter high-quality instruction-following data according to question type, correctness, and other indicators.
Similarly, LLaVA-Med~\citep{llava-med2023arxiv}, also based on the PMC dataset, uses preset prompts to guide GPT-4 to generate multi-round of conversations.
OphGLM~\citep{ophglm2023arxiv} collects corresponding images and subject knowledge for ophthalmic examination scenarios, uses predefined prompts combined with ChatGPT to mimic real-world doctor-patient question-answer sessions to generate multi-round instruction conversations, and designs three rounds of quality control strategies.
GPT4Tools~\citep{gpt4tools2023arxiv} proposes a set of tool-related instruction datasets for the use requirements of various vision tools.
mPLUG-DocOwl~\citep{mplugdoc2023arxiv} generates a document instruction dataset by integrating five document-related tasks with pure text and general vision-language instruction data for document understanding tasks.
PointLLM~\citep{pointllm2023arxiv} has proposed a complete set of point cloud instruction data based on GPT-4 for point cloud processing.

\subsubsection{Data Mixing}\label{sec:data_mix}

Meanwhile, there is a class of MLLMs, e.g., mPLUG-Owl~\citep{mplug2023arxiv}, X-LLM~\citep{xllm2023arxiv}, PandaGPT~\citep{pandagpt2023arxiv}, Video-LLaMA~\citep{videollama2023arxiv}, MultiModal-GPT~\citep{multimodalgpt2023arxiv}, LaVIN~\citep{lavin2023arxiv}, BuboGPT~\citep{bubo2023arxiv}, ImageBind-LLM~\citep{imagebind2023arxiv}, BLIVA~\citep{bliva2023arxiv}, Qwen-VL~\citep{qwen2023arxiv}, mPLUG-Owl2~\citep{mplugowl22023arxiv} that do not construct new instruction data independently, but mix existing VLIT datasets and task data.
In addition, there are vast models that mix existing VLIT data with self-constructed datasets in order to expand the scale of VLIT data. 
Please refer to Table~\ref{tab:mllm} for details.

\subsection{Construction Tools}\label{sec:const_tools}

Besides, based on the existing mature experience, some relatively complete construction tools have been proposed to realize the end-to-end VLIT data construction.
These frameworks usually include considerations and optimizations for important steps such as data collection and filtering.

Specifically, M$^3$IT~\citep{m3it2023arxiv} proposes a complete instruction-following data construction pipeline, which first allocates a selectable instruction pool for 6 major task types, integrates region and context information into task data, and performs quality checks manually.
Sythus~\citep{mimic2023arxiv} is a pipeline that automatically generates high-quality instruction-response pairs based on visual content. It generates a massive amount of instruction-following data based on ChatGPT (namely MIMIC-IT) with two scenarios as targets: general scene understanding and egocentric view understanding.
MULTIINSTRUCT~\citep{multiinstruct2022arxiv} designs a three-step instruction template design and verification process involving multiple human annotators to generate high-quality instructions, and combined with ten visual tasks to generate a large amount of instruction-formatted data.
Polite Flamingo~\citep{pf2023arxiv} designs and trains an instruction-response rewriter based on existing VLIT data, and further rewrites a large amount of publicly available multi-modal dataset into large-scale instruction-following data.
ASM~\citep{as2023arxiv} collects common open-source datasets to meet the demand for understanding fine-grained information in visual signals, forming billion-level region-oriented semantic labels, detail descriptions, and question-answer data.
Cheetor~\citep{cheetor2023arxiv} constructs an image-text interleaved instruction dataset I4, covering 7 major vision-language tasks, and generates standard instruction data triplets based on the original annotated data.
VIGC~\citep{vigc2023arxiv} proposes a vision-language instruction generation and correction framework, which uses an iterative update mechanism and multi-modal LLM to generate instruction-following data, achieving the effect of reducing hallucinations and enhancing diversity.
MLLM-DataEngine~\citep{mllm-de2023arxiv} considers the three stages of data generation, model training, and evaluation as a single round, and guides the next round of data collection (adaptive sampling module) based on the analysis of model deficiencies. At the same time, in the generation of instruction data, it combines human and GPT-4 to optimize the overall quality of instruction data through multi-round interaction.
CIEM~\citep{ciem2023arxiv} proposes a solution to alleviate the hallucination problem of LLMs by automatically generating high-quality fact/contrast question-answer pairs and the corresponding tuning strategy.

However, these methods generally only perform relatively simple filtering of the generated VLIT data based on subjective experience, and do not actually quantify the changes in quality before and after filtering.
At the same time, the performance improvement brought by data filtering has not been correlated with the performance changes of MLLM.
Therefore, it is still unclear how to improve the quality of VLIT and thereby improve the performance of tuned MLLMs.

\subsection{Analysis}

As the instruction tuning stage has become a necessary fine-tuning stage in MLLMs, vast VLIT datasets have been proposed. 
These datasets are extremely large in scale, covering a massive number of visual tasks, and rely on the powerful capabilities of LLMs to make the corresponding instruction content more diverse. 
MLLMs have also shown in evaluations that instruction tuning based on such datasets does indeed bring corresponding performance improvements. 
However, there are two main problems in the construction of the current VLIT dataset.
\begin{itemize}
    \item First of all, all existing VLIT data construction methods are based on intuition and some scattered unverified practical experience, and lack reasonable, reliable, and systematic construction principles to guide the construction of VLIT data.
    \item Secondly, the current instruction data filtering strategy is still very rough and cannot quantitatively and qualitatively evaluate a single data sample and the overall data distribution. As a result, the existing VLIT data is generally very large and noisy, which greatly affects the downstream performance and tuning efficiency of MLLMs.
\end{itemize}

